Reversing the Forget-Retain Objectives: An Efficient LLM Unlearning Framework from Logit Difference

As Large Language Models (LLMs) demonstrate extensive capability in learning from documents, LLM unlearning becomes an increasingly important research area to address concerns of LLMs in terms of privacy, copyright, etc. A conventional LLM unlearning task typically involves two goals: (1) The target LLM should forget the knowledge in the specified forget documents, and (2) it should retain the other knowledge that the LLM possesses, for which we assume access to a small number of retain documents. To achieve both goals, a mainstream class of LLM unlearning methods introduces an optimization framework with a combination of two objectives - maximizing the prediction loss on the forget documents while minimizing that on the retain documents, which suffers from two challenges, degenerated output and catastrophic forgetting. In this paper, we propose a novel unlearning framework called Unlearning from Logit Difference (ULD), which introduces an assistant LLM that aims to achieve the opposite of the unlearning goals: remembering the forget documents and forgetting the retain knowledge. ULD then derives the unlearned LLM by computing the logit difference between the target and the assistant LLMs. We show that such reversed objectives would naturally resolve both aforementioned challenges while significantly improving the training efficiency. Extensive experiments demonstrate that our method efficiently achieves the intended forgetting while preserving the LLM's overall capabilities, reducing training time by more than threefold. Notably, our method loses 0% of model utility on the ToFU benchmark, whereas baseline methods may sacrifice 17% of utility on average to achieve comparable forget quality. Our code will be publicly available at https://github.com/UCSB-NLP-Chang/ULD.

==> sections/98_impact_limitation.tex <==
\section{Broad Impacts} \label{sec:impact}

Our work proposes an efficient and effective LLM unlearning framework \algnamens, which has a broad impact on improving privacy and data leakage issues in LLM usage, making LLMs safer and more reliable in practical application. 
Unlike existing unlearning methods that may sacrifice the LLM's overall capability to achieve the desired unlearning. Our work does not change the parameters of original LLM and introduces an assistant LLM to help build the unlearned LLM via logit subtraction operation. This solves the common challenges of conventional unlearning objectives that may harm the retention of knowledge and improves the efficiency of the unlearning process. 

We also note that the proposed framework is not limited to the LLM unlearning. Similar to previous works in LLM decoding literature~\cite{chuang2023dola, li2022contrastive}, we plan to explore applying our method to other tasks like sentiment-controlled text generation, knowledge editing, and improving LLM's factuality.


\section{Limitations}\label{sec:limitation}

While \algname enhances the training efficiency and stability of the unlearning process, our method involves an assistant LLM during inference, which may lead to higher inference latency. However, this increase can be mitigated by parallelizing the computations of the assistant LLM and the original LLM. 
Additionally, although forget data augmentation is crucial for improving the unlearn performance for \algnamens, creating appropriate augmentations for different datasets can be challenging. We plan to explore the automatic construction of optimal forget data construction in future work.






